SymBa: Symbolic Backward Chaining for Structured Natural Language Reasoning

To improve the performance and explainability of LLM-based natural language reasoning, structured reasoning can be applied to generate explicitly structured proofs. Among different methods for structured reasoning, we specifically focus on backward chaining, where the proof goal is recursively decomposed to subgoals by searching and applying rules. We argue that current LLM-based backward chaining systems (e.g. Least-to-most prompting and LAMBADA) are incomplete, as they omit crucial algorithmic components identified from the classic backward chaining algorithm in computational logic (SLD Resolution). To this end, we propose a novel backward chaining system, SymBa (Symbolic Backward Chaining), which integrates a symbolic solver and an LLM. In SymBa, the solver controls the proof process, and the LLM is only called when the solver requires new information to complete the proof. Empowered by completeness, SymBa achieves a significant improvement in seven deductive, relational, and arithmetic reasoning benchmarks compared to the baselines.

==> content/A3_prompts.tex <==
\section{Prompts}

In this section, we provide prompts used for single-step statement generation in \ours \ for each task. Note that for CLUTRR and ECtHR, we do not need Rule Search/Translation because all necessary rules are provided by the corresponding expert system. Furthermore, we will release the prompts (Standard prompting, Chain-of-thought prompting, Least-to-most prompting, and LAMBADA) upon acceptance.

\subsection{ProofWriter family}

\subsubsection{Fact Search}

\rule{\columnwidth}{0.4pt}\\
\small
Find a single fact from the context that is applicable to the query, one per each line.\\
\\
Example 1\\
Context: The bear chases the mouse. The cat is big. The dog is rough. The mouse likes the cat.\\
Query: likes(mouse, \_)\\
Applicable fact: The mouse likes the cat.\\
\\
Example 2\\
Context: Anne is round. Erin is furry. Fiona is blue.\\
Query: is(erin, round)\\
Applicable fact: No applicable fact.\\
\\
Example 3\\
Context: The bald eagle chases the dog. The dog chases the lion. The lion eats the bald eagle.\\
Query: chases(\_, dog)\\
Applicable fact: The bald eagle chases the dog.\\
\\
Example 4\\
Context: \{facts\}\\
Query: \{query\}\\
Applicable fact:\\
\normalsize
\rule{\columnwidth}{0.4pt}
 
\subsubsection{Rule Search}

\rule{\columnwidth}{0.4pt}\\
\small
Find rules from the context that is applicable to the query, one per each line.\\
\\
Example 1\\
Context: If the dog is cold and the dog likes the cat then the cat is cold. If someone chases the cat and they like the bear then the cat likes the mouse. If someone likes the bear and the bear does not chase the cat then the bear likes the mouse. If someone is cold and young then they chase the mouse. If someone likes the mouse then they like the cat. If someone is big and not young then they like the bear.\\
Query: likes(\_, mouse)\\
Applicable rules: If someone chases the cat and they like the bear then the cat likes the mouse.\\
If someone likes the bear and the bear does not chase the cat then the bear likes the mouse.\\
\\
Example 2\\
Context: All furry people are round. If someone is round and furry then they are green.\\
Query: is(eric, round)\\
Applicable rules: All furry people are round.\\
\\
Example 3\\
Context: If someone chases the bald eagle and the bald eagle is not cold then they eat the bald eagle. If the lion does not eat the dog then the dog chases the bald eagle.\\
Query: eats(mouse, bald\_eagle)\\
Applicable rules: If someone chases the bald eagle and the bald eagle is not cold then they eat the bald eagle.\\
\\
Example 4\\
Context: \{rules\}\\
Query: \{query\}\\
Applicable rules:\\
\normalsize
\rule{\columnwidth}{0.4pt}

\subsubsection{Fact Translation}

\rule{\columnwidth}{0.4pt}\\
\small
Example 1\\
Query: likes(mouse, \_)\\
Fact: The mouse likes the cat.\\
Statement: likes(mouse, cat).\\
\\
Example 2\\
Query: is(erin, red)\\
Fact: Erin is round.\\
Statement: is(erin, round).\\
\\
Example 3\\
Query: chases(\_, lion)\\
Fact: The bald eagle chases the dog.\\
Statement: chases(bald\_eagle, dog).\\
\\
Example 4\\
Query: \{query\}\\
Fact: \{fact\}\\
Statement:\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsubsection{Rule Translation}

\rule{\columnwidth}{0.4pt}\\
\small
Example 1\\
Query: likes(\_, bear)\\
Rule: If someone likes the bear and the bear does not chase the cat then the bear likes the mouse.\\
Statement: likes(bear, mouse) :- likes(X, bear), not chases(bear, cat).\\
\\
Example 2\\
Query: is(erin, furry)\\
Rule: All furry people are round.\\
Statement: is(X, round) :- is(X, furry).\\
\\
Example 3\\
Query: eats(rabbit, bald\_eagle)\\
Rule: If someone chases the bald eagle and the bald eagle is not cold then they eat the bald eagle.\\
Statement: eats(X, bald\_eagle) :- chases(X, bald\_eagle), not is(bald\_eagle, cold).\\
\\
Example 4\\
Query: \{query\}\\
Rule: \{rule\}\\
Statement:\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsection{GSM8k}

\subsubsection{Fact Search}

\rule{\columnwidth}{0.4pt}\\
\small
Find a single fact from the context that is applicable to the query, one per each line.\\
\\
Example 1\\
Context: Julie is reading a 120-page book. Yesterday, she was able to read 12 pages and today, she read twice as many pages as yesterday. If she wants to read half of the remaining pages tomorrow, how many pages should she read?\\
Query: answer(\_)\\
Applicable fact: The value of query: answer(\_) is not directly given in the passage.\\
\\
Example 2\\
Context: Mark has a garden with flowers. He planted plants of three different colors in it. Ten of them are yellow, and there are 80\% more of those in purple. There are only 25\% as many green flowers as there are yellow and purple flowers. How many flowers does Mark have in his garden?\\
Query: number\_of\_yellow\_flowers(\_)\\
Applicable fact: The value of query: number\_of\_yellow\_flowers(\_) is directly given as 10.\\
\\
Example 3\\
Context: Ursula bought five hot dogs at \$1.50 each and three salads at \$2.50 each. If she had two \$10 bills, how much change did she get back?\\
Query: changes\_ursula\_got\_back(\_)\\
Applicable fact: The value of query: changes\_ursula\_got\_back(\_) is not directly given in the passage.\\
\\
Example 4\\
Context: A truck driver has to spend \$2 per gallon of gas. She can drive 10 miles per gallon. She drives at a rate of 30 miles per hour. If she is paid \$.50 per mile, how much money does she make if she drives for 10 hours?\\
Query: driver\_speed\_in\_mph(\_)\\
Applicable fact: The value of query: driver\_speed\_in\_mph(\_) is directly given as 30 mph.\\
\\
Example 5\\
Context: Building A has 4 floors, which is 9 less than Building B. Building C has six less than five times as many floors as Building B. How many floors does Building C have?\\
Query: floors\_of\_building\_A(\_)\\
Applicable fact: The value of query: floors\_of\_building\_A(\_) is directly given as 4.\\
\\
Example 6\\
Context: \{facts\}\\
Query: \{query\}\\
Applicable fact:\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsubsection{Rule Search}

\rule{\columnwidth}{0.4pt}\\
\small
Find rules from the context that is applicable to the query, one per each line.\\
\\
Example 1\\
Context: Julie is reading a 120-page book. Yesterday, she was able to read 12 pages and today, she read twice as many pages as yesterday. If she wants to read half of the remaining pages tomorrow, how many pages should she read?\\
Query: answer(\_)\\
Applicable rules: The value of query: answer(\_) can be calculated by "the number of remaining pages" * 0.5.\\
\\
Example 2\\
Context: Mark has a garden with flowers. He planted plants of three different colors in it. Ten of them are yellow, and there are 80\% more of those in purple. There are only 25\% as many green flowers as there are yellow and purple flowers. How many flowers does Mark have in his garden?\\
Query: number\_of\_green\_flowers(\_)\\
Applicable rules: The value of query: number\_of\_green\_flowers(\_) can be calculated as "total number of yellow and purple flowers" * 0.25.\\
\\
Example 3\\
Context: Ursula bought five hot dogs at \$1.50 each and three salads at \$2.50 each. If she had two \$10 bills, how much change did she get back?\\
Query: total\_price\_of\_hot\_dogs(\_)\\
Applicable rules: The value of query: total\_price\_of\_hot\_dogs(\_) can be calculated as "the number of hot dogs Ursula bought" * "the price of single hot dog in dollars".\\
\\
Example 4\\
Context: A truck driver has to spend \$2 per gallon of gas. She can drive 10 miles per gallon. She drives at a rate of 30 miles per hour. If she is paid \$.50 per mile, how much money does she make if she drives for 10 hours?\\
Query: money\_driver\_made\_by\_driving\_10\_hours(\_)\\
Applicable rules: The value of query: money\_driver\_made\_by\_driving\_10\_hours(\_) can be calculated as "the total money spent on gas in dollars" - "the total amount of money driver is paid in dollars".\\
\\
Example 5\\
Context: Building A has 4 floors, which is 9 less than Building B. Building C has six less than five times as many floors as Building B. How many floors does Building C have?\\
Query: floors\_of\_building\_C(\_)\\
Applicable rules: The value of query: floors\_of\_building\_C(\_) can be calculated as 5 * "floors of Building B" - 6.\\
\\
Example 6\\
Context: \{facts\}\\
Query: \{query\}\\
Applicable rules:\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsubsection{Fact Translation}

\rule{\columnwidth}{0.4pt}\\
\small
Example 1\\
Query: answer(\_)\\
Fact: answer(\_) is not directly given in the passage.\\
Statement: not answer.\\
Example 2\\
Query: number\_of\_green\_flowers(\_)\\
Fact: The value of query: number\_of\_green\_flowers(\_) is not directly given in the passage.\\
Statement: not number\_of\_yellow\_flowers.\\
\\
Example 3\\
Query: money\_ursula\_had\_initially(\_)\\
Fact: The value of query: money\_ursula\_had\_initially(\_) is directly given as \$20.\\
Statement: money\_ursula\_had\_initially(20).\\
\\
Example 4\\
Query: total\_money\_spend\_in\_gas(\_)\\
Fact: The value of query: driver\_speed\_in\_mph(\_) is directly given as 30 mph.\\
Statement: driver\_speed\_in\_mph(30).\\
\\
Example 5\\
Query: floors\_of\_building\_C(\_)\\
Fact: The value of query: floors\_of\_building\_A(\_) is directly given as 4.\\
Statement: The value of query: floors\_of\_building\_A(4).\\
\\
Example 6\\
Query: \{query\}\\
Fact: \{fact\}\\
Statement:\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsubsection{Rule Translation}

\rule{\columnwidth}{0.4pt}\\
\small
Example 1\\
Query: answer(\_)\\
Rule: The value of query: answer(\_) can be calculated by "the number of remaining pages" * 0.5.\\
Statement: answer(X) :- number\_of\_remaining\_pages(A), X = A / 2.\\
\\
Example 2\\
Query: number\_of\_green\_flowers(\_)\\
Rule: The value of query: number\_of\_green\_flowers(\_) can be calculated as "total number of yellow and purple flowers" * 0.25.\\
Statement: number\_of\_green\_flowers(X) :- number\_of\_purple\_and\_yellow\_flowers(A), X = A * 0.25.\\
\\
Example 3\\
Query: total\_price\_of\_hot\_dogs(\_)\\
Rule: The value of query: total\_price\_of\_hot\_dogs(\_) can be calculated as "the number of hot dogs Ursula bought" * "the price of single hot dog in dollars".\\
Statement: total\_price\_of\_hot\_dogs(X) :- number\_of\_hotdogs\_ursula\_bought(A), price\_of\_single\_hotdog(B), X = A * B.\\
\\
Example 4\\
Query: money\_driver\_made\_by\_driving\_10\_hours(\_)\\
Rule: The value of query: money\_driver\_made\_by\_driving\_10\_hours(\_) can be calculated as "the total money spent on gas in dollars" - "the total amount of money driver is paid in dollars".\\
Statement: money\_driver\_made\_by\_driving\_10\_hours(X) :- total\_money\_spent\_on\_gas(A), total\_amount\_of\_money\_driver\_is\_paid(B), X = B - A.\\
\\
Example 5\\
Query: floors\_of\_building\_C(\_)\\
Rule: The value of query: floors\_of\_building\_C(\_) can be calculated as 5 * "floors of Building B" - 6.\\
Statement: floors\_of\_building\_C(X) :- floors\_of\_building\_B(A), X = (5 * A) - 6.\\
\\
Example 6\\
Query: \{query\}\\
Rule: \{rule\}\\
Statement:\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsection{CLUTRR-TF}

\subsubsection{Fact Search}

\rule{\columnwidth}{0.4pt}\\
\small
Find a single fact from the context that is applicable to the query, one per each line.\\
\\
Example 1\\
Context: [George] was proud to attend [Andrea]'s graduation. He was very proud to have raised her into a successful young adult. [John] went shopping with his wife [Andrea].\\
Query: isRelationOf(george, father, \_)\\
Applicable fact: George is the father of Andrea.\\
\\
Example 2\\
Context: [Carrie] was worried about her graduation party. Her mother [Cindy] had turned up earlier that day, but her brother [Wayne] was still missing. [Lena] is getting married. She is looking forward to her sister, [Cindy], attending. They have n't seen each other since [Cindy] relocated to California with her husband 3 years ago.\\
Query: isRelationOf(carrie, daughter, \_)\\
Applicable fact: Carrie is the daughter of Cindy.\\
\\
Example 3\\
Context: [Shantel] and her husband [Harold] took her son [Pedro] to the store to pick out some sweets after dinner. [Dorothy] and her daughter [Heather] went out to dinner. [Dorothy] went with her husband [Pedro] to get a nice dinner for their anniversary.\\
Query: isRelationOf(heather, granddaughter, \_)\\
Applicable fact: Heather is the daughter of Dorothy.\\
\\
Example 4\\
Context: \{facts\}\\
Query: \{query\}\\
Applicable fact:\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsubsection{Rule Search}

\rule{\columnwidth}{0.4pt}\\
\small
print "No applicable rule."\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsubsection{Fact Translation}

\rule{\columnwidth}{0.4pt}\\
\small
Example 1\\
Query: isRelationOf(george, father, \_).\\
Fact: George is the father of Andrea.\\
Statement: isRelationOf(george, father, andrea).\\
\\
Example 2\\
Query: isRelationOf(cindy, sister, \_)\\
Fact: Cindy is the mother of Carrie.\\
Statement: isRelationOf(cindy, mother, carrie).\\
\\
Example 3\\
Query: isRelationOf(heather, daughter, \_)\\
Fact: Heather is the daughter of Dorothy.\\
Statement: isRelationOf(heather, daughter, dorothy).\\
\\
Example 4\\
Query: \{query\}\\
Fact: \{fact\}\\
Statement:\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsubsection{Rule Translation}

\rule{\columnwidth}{0.4pt}\\
\small
print "No applicable rule."\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsection{ECtHR Article 6}

\subsubsection{Fact Search}

\rule{\columnwidth}{0.4pt}\\
\small
Find a single fact that is applicable to the query, one per each line.\\
\\
Example 1\\
Context: (Information regarding the case) \\
Query: checkIf("some question", \_)\\
Applicable fact: Since (summary of the relevant facts to the question), "some question" is seriously violated/not seriously violated. (Note: you must choose only one.)\\
\\
Example 2\\
Context: \{facts\}\\
Query: \{query\}\\
Applicable fact:\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsubsection{Rule Search}

\rule{\columnwidth}{0.4pt}\\
\small
print "No applicable rule."\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsubsection{Fact Translation}

\rule{\columnwidth}{0.4pt}\\
\small
Example 1\\
Query: checkIf("some question", \_)\\
Fact: Since (summary of the relevant facts), "some question" is not\_seriously\_violated.\\
Statement: checkIf("some question", not\_seriously\_violated). (Note: the second argument must be one of seriously\_violated or not\_seriously\_violated.)\\
\\
Example 2\\
Query: \{query\}\\
Fact: \{fact\}\\
Statement:\\
\normalsize\rule{\columnwidth}{0.4pt}

\subsubsection{Rule Translation}

\rule{\columnwidth}{0.4pt}\\
\small
print "No applicable rule."\\
\normalsize\rule{\columnwidth}{0.4pt}


==> content/A4_error_analysis.tex <==
\section{Error analysis}
\label{sec:appendix_error}

In this section, we further provide details of the error analysis introduced in Section \ref{sec:error}.

\subsection{Qualitative analysis}

\textbf{ProofWriter} The Rule Search module often fails to retrieve a unifying rule if the rule is not bound, as quantitatively analyzed in Section \ref{sec:error}. For instance, the model failed to find the unbound rule "\textit{If something is round then it chases the dog.}" from the query $\texttt{chases}(\texttt{tiger}, \texttt{dog)}$.

\textbf{Birds-Electricity} Errors from Birds-Electricity are mostly due to undesired common sense reasoning; \textit{e.g.} "\textit{The switch is on.}" is falsely retrieved from the query $\texttt{runs\_through}(\texttt{current}, \texttt{switch})$. While these two facts do not relate with each other formally, the former often implies the latter in daily contexts.

\textbf{CLUTRR} Similar to ProofWriter, Search-Miss is the most dominant error type observed in CLUTRR. However, the context of CLUTRR only contains ground facts and no unground rules. The major cause of error in CLUTRR is that the model has to infer the \textit{reverse} of the relationship exposed in the context. For example, the model could not relate $\texttt{isRelationTo}(lisa, daughter, \_)$" to \textit{[Lisa] and [Roger] did the Father daughter dance at the recital.}".

\textbf{GSM8k} In GSM8k dataset, the model suffers from multiple possible interpretations of predicate names generated by its own, \textit{e.g.} $\texttt{cost\_of\_sale\_unit}$ can be interpreted as "the price of single yogurt" or "the price of 4 yogurts" in "\textit{They are currently on sale at 4 yogurts for \$5.00.}". Also, it often fails to formulate non-arithmetic operations such as maximum function correctly. If the answer is the maximum value of \texttt{thursday\_revenue} and \texttt{friday\_revenue}, an acceptable statement example would be \texttt{answer$(X)$ :- thursday\_revenue$(A), $friday\_revenue$(B), A > B, X = A$.} and the other way around ($B > A, X=B$), but the model has generated an ill-formed code as \texttt{answer$(X)$ :- thursday\_revenue$(A), $friday\_revenue$(B), X = A > B$.}

% \textbf{ECtHR} In ECtHR, the model often misjudges that a random, irrelevant fact is somehow related to the query. For instance, the model has concluded that the criteria "\textit{Evidence is fairly obtained and administered}" was seriously violated from the fact that "\textit{The defence had made excessive use of their right ... and had filed around 500 applications for the taking of evidence ... that was impossible to obtain, ...}". However, as '\textit{the defence}' refers to the applicants of this ECtHR case, this fact only implies that the applicant is responsible for the delay of the questioned case, not that evidence was unfairly obtained or administered.\footnote{The case exemplified here is Demjanjuk v. Germany, application number 24247/15.}

\subsection{Quantitative analysis}

In this section, we provide details about the experiment presented in Section \ref{sec:error}, which tests the effects of bound and unbound rules.

We use the original ProofWriter test set (closed-world assumption). A rule is classified as bound (unbound) if it does not include (does include) the word 'someone' or 'something'. For bound rules, the corresponding query is identical to the rule head. For bound rules, as the rule head contains variables, we substitute the variable with a random entity name sampled from the dataset. Among these query-rule pairs, we filter out cases where the query matches two or more rules in the context. Finally, we randomly sample 30 context-query-rule triplets for each context length (number of facts and rules in the statement) from 15 to 25 and whether the rule is bound, resulting in 660 examples.

Since falsely retrieved rules that do not unify with the query are automatically filtered out by the Symbolic Validation module, we select recall as the core metric over precision and F1 score. The results presented in Figure \ref{fig:errorheatmap} also support this claim, as relatively few Search-Hallucination errors are observed from the ProofWriter dataset.

The recall score reported in Figure \ref{fig:errorquant} averages 330 samples for bound/unbound rules. The full results are plotted in Figure \ref{fig:errorquant-appendix}, where the context length and the recall score demonstrates a relatively minor negative correlation compared to the boundness of the target rule.

% \begin{figure}[ht]
%     \centering
%     \includesvg[width=\columnwidth]{figures/vectors/errorquant_appendix.svg}
%     \caption{Recall of Rule Search module in ProofWriter plotted with the number of statements (facts and rules) in the context. Each data point represents the average of 30 samples.}
%     \label{fig:errorquant-appendix}
% \end{figure}

Besides our experiment on the type of rules (bound / not bound), \citet{kazemi-etal-2023-lambada} has reported that the accuracy of the Fact Check module, which directly corresponds to \ours's Fact Search module, is strongly dependent on the model size. Applying an external search module specialized for searching unifying rules rather than using LLMs could significantly increase the performance. However, we leave this direction as future work.

==> table/table_llm.tex <==
\begin{table}[ht]
    \small
    \centering
    \begin{tabular}{l|c|c|c}
         \multicolumn{1}{c|}{Model} & Provider & Open? & Release ver. \\
         \hline \hline
         GPT-4 Turbo & OpenAI & N & 11/04/2023 \\
         Claude 3 Sonnet & Anthropic & N & 02/29/2024 \\
         LLaMa 3 70B & Meta & Y & 04/18/2024
    \end{tabular}
    \caption{Brief information of LLMs applied in this study. \textit{Release date} column refers to the version of the specific checkpoints or API endpoints used for the experiments.}
    \label{tab:llm}
\end{table}

